DT-RAID: A Software-Defined Tiered RAID Architecture for Heterogeneous SSDs

The rapid proliferation of cloud and AI-driven workloads has led to increasingly complex requirements for modern storage subsystems. To meet these demands, SSD controller architectures have evolved into a fragmented landscape, offering tiers of drive types optimized for endurance, performance, or capacity. More recently, SSDs have begun to differentiate regions within the same device, enabling intra-drive heterogeneity. However, integrating such heterogeneity into the existing storage stack with minimal disruption remains challenging. In this paper, we argue that storage middleware, such as RAID, is an effective control layer to address these integration challenges. We present DT-RAID, an intra-drive heterogeneity-aware RAID architecture designed for emerging SSDs. DT-RAID monitors stripe-level I/O access patterns and makes online placement decisions without requiring application modifications. It employs a lightweight heat-tracking mechanism to dynamically place frequently accessed (hot) stripes onto the higher-performance, higher-endurance tier. Using simulations based on SNIA MSR enterprise I/O traces, we demonstrate that DT-RAID improves modeled I/O performance by up to $6.8\times$ under greater tier asymmetry and extends normalized lifespan by up to $20.9\times$ compared to uniform RAID deployments.

==> src/v4/scratch_pad.tex <==

% 260316-CC: For your reference, I have rearranged the materials of several paragraphs. Meanwhile, I try to strengthen the connection for the contents of the previous 3 paragraphs.  

% \IEEEPARstart{M}{odern} data-intensive services must simultaneously deliver high I/O performance, low tail latency, and strong data reliability, while operating under increasingly diverse and rapidly evolving workload conditions~\cite{li2020cloudblock,10.1145/3297663.3310302,ZhichaoCao2020RocksDBworkloads,berg2020cachelib,tang2023cloudonomics}. In large-scale infrastructures, the same storage backend may concurrently support lakehouse platforms with long-running batch and streaming pipelines, transactional database and key--value store services, and emerging AI training and inference workloads~\cite{Dong2024CloudNativeDatabases,Xue2024LakehouseScale,Hu2024CharLLMinDatacenter}. These systems require storage not only to provide high bandwidth and low latency, but also to tolerate device failures without sacrificing availability. As a result, \emph{Redundant Array of Independent Disks} (RAID) remains a widely deployed mechanism for combining multiple drives to improve both performance and reliability. At the same time, NAND-based Solid-State Drives (SSDs) have become the dominant medium in performance-critical storage systems, making RAID over SSDs a foundational building block in modern data infrastructure.

% To meet increasingly diverse workload requirements, the SSD ecosystem has evolved beyond uniform device designs. Vendors now offer SSDs spanning low-latency, balanced enterprise, and high-density capacity-oriented operating points~\cite{KIOXIAFL6Datasheet,SolidigmD7P5810Brief,PhisonPascariX200Z}. More importantly, recent designs increasingly integrate multiple flash technologies, such as SLC, TLC, and QLC, within a single device. This \emph{intra-device heterogeneity} creates internal tiers with distinct latency, endurance, and capacity characteristics, opening new opportunities for differentiated placement and resource management~\cite{Radu2019HybridFlashCTRL}. Although such heterogeneity is still largely hidden behind today’s block interface, emerging host-managed storage interfaces and recent SSD proposals make host-visible control increasingly plausible~\cite{Boukhobza2025HostSideFlash,2025MixedModeSSD,2025scalaafa-journal,2025KVSSD_park,kang2014multistreamssd,NVMeNVMCommandSet12_FDP,NVMeZNSCommandSet12}. These developments suggest that future SSDs may expose multiple internal tiers that the host can manage explicitly, rather than forcing all data to be treated uniformly.

% A natural question, then, is where such intra-device heterogeneity should be managed. One possibility is to push placement decisions into applications, but this requires per-application modification, incurs significant engineering overhead, and tightly couples software to hardware-specific features~\cite{purandare2025valetefficientdataplacement}. Another possibility is to rely on SSD-internal tiering, but device-managed policies lack system-level visibility across concurrent workloads, cannot directly reason about end-to-end redundancy semantics, and remain constrained by controller resources and internal heuristics~\cite{Yoo2020SLCCache-tierbackdraw,Boukhobza2025HostSideFlash}. We instead argue that the RAID layer is the most practical control point for exploiting host-visible SSD heterogeneity. RAID already preserves the standard block interface expected by applications, has visibility into access patterns across devices, and directly manages data and parity placement. This combination allows RAID to exploit tier asymmetry without requiring application changes or deep SSD-internal modifications.

% This observation is particularly important for parity-based RAID systems. In RAID-5 and related designs, maintaining redundancy consistency introduces extra reads and writes beyond user I/O. These parity-maintenance operations are not evenly distributed over time: under skewed and update-intensive workloads, a small subset of stripes can repeatedly trigger read--modify--write or related parity-consistent updates. As a result, the cost of a write in RAID is determined not only by the user request itself, but also by which stripe is updated, how often that stripe is revisited, and where its data and parity reside. Once SSDs expose heterogeneous internal tiers, stripe placement becomes cost-critical: latency can be bounded by the slowest tier on the update path, while parity-induced write amplification can disproportionately consume the endurance budget of less durable tiers. In other words, parity maintenance turns tier asymmetry into a RAID-level placement problem rather than a purely device-local optimization opportunity.

% Existing RAID research does not fully address this problem. Prior work on all-flash RAID primarily assumes homogeneous SSD arrays and focuses on removing software bottlenecks such as lock contention, limited parallelism, and parity-processing overhead~\cite{2022scalaraid,Shu2023dRAID}. Other efforts consider heterogeneity across drives, or use fast flash regions as transient staging buffers, but they do not fundamentally revisit the RAID abstraction itself as a placement layer for persistent data and parity under intra-device tier asymmetry. As a result, current RAID designs still largely treat each SSD as a uniform block device, even when the underlying flash organization is not uniform. This leaves an important question unanswered: if SSDs expose performance- and capacity-optimized internal tiers to the host, how should RAID place data and parity across those tiers to improve both performance and lifetime?

% In this paper, we answer this question by studying how RAID can exploit intra-device heterogeneity through stripe-aware placement. We show that parity-based redundancy makes stripe-level placement a first-order concern in heterogeneous SSD environments, especially under skewed updates. To capture this effect, we develop a lightweight heat-tracking mechanism that monitors stripe-level update intensity and enables RAID to distinguish between cold and hot stripes. Building on this mechanism, we propose \emph{DT-RAID} (Dual-Tier RAID), a RAID architecture that manages data and parity placement across performance- and capacity-optimized tiers within an SSD array. We focus on a dual-tier setting because it captures the fundamental performance--capacity--endurance tradeoff while remaining sufficiently general to represent emerging heterogeneous SSD designs.

% Because commodity SSDs do not yet widely expose such host-visible internal tiers, we develop a trace-driven RAID simulation platform to explore this design space. Using enterprise I/O traces from the SNIA IOTTA repository~\cite{msr_iotta}, we show that DT-RAID improves throughput by up to 4.83$\times$ and reduces device wear by up to 20$\times$, while incurring only modest capacity overhead.


%shorten KCC 0326
% \Cref{fig:io_acceleration_8disk_raid5} reports the normalized I/O acceleration, with ST normalized to \(1\times\). Across workloads, DT-S improves performance moderately, raising acceleration to 1.19$\times$--1.47$\times$ by redirecting parity-related flash activity to the performance tier. DT-D delivers substantially larger gains, increasing acceleration to 1.75$\times$--3.10$\times$ through heat-guided whole-stripe migration. This trend is consistent with \Cref{fig:flash_breakdown_8disks_raid5}: DT-D shifts a much larger fraction of flash activity from the capacity tier to the performance tier. Migration overhead is explicitly included in the accounting, and for the evaluated workloads, relocation is dominated by promotions while demotions are rare.

%% Evaluation Performance.
% \Cref{fig:io_acceleration_8disk_raid5} reports the resulting normalized I/O acceleration, with ST normalized to \(1\times\). Across all workloads, DT-S consistently improves effective I/O performance over ST by steering parity-related flash activity to the performance tier. The resulting acceleration ranges from \(1.21\times\) to \(1.54\times\). These gains show that even static parity placement can reduce the effective flash service cost associated with parity maintenance.

% DT-D further improves performance by relocating hot stripes to the performance tier based on the cost-aware heat metric. Under DT-D, the normalized I/O acceleration increases to \(2.17\times\) for \texttt{hm\_0}, \(4.44\times\) for \texttt{proj\_0}, \(4.55\times\) for \texttt{prxy\_0}, and \(4.83\times\) for \texttt{prxy\_1}. Compared with DT-S, these gains are substantially larger across all workloads, especially for \texttt{proj\_0}, \texttt{prxy\_0}, and \texttt{prxy\_1}. This trend is consistent with the tier-level flash breakdown in \Cref{fig:flash_breakdown_8disks_raid5}: DT-D shifts a much larger fraction of both reads and writes from the capacity tier to the performance tier. In our experiments, migration overhead is explicitly accounted for as additional read-plus-program activity, and the observed relocation is dominated by promotions, while demotions are rare for the evaluated workloads.

%% Lifespan from Radu
% H3 examines whether tier-aware stripe placement improves array lifetime, and how strongly this benefit depends on endurance asymmetry between the performance and capacity tiers. We estimate lifetime consumption using flash block erase counts and report the \emph{normalized lifespan improvement} relative to ST RAID. To stress-test this effect, we sweep the endurance ratio between the performance tier and the capacity tier from 1:1 to 100:1 under RAID-5 (8-disk, 4\,KB) across four workloads. \Cref{fig:flash_lifespan_improvement_raid5_8disk_4k} summarizes the results.

%% I/O acceleration
Having shown that DT-RAID can redirect a large fraction of flash activity to the performance tier with bounded overhead, we next ask whether this steering translates into a lower effective flash service cost. Because our framework isolates RAID-layer effects rather than full end-to-end system latency, we evaluate performance using a flash-time-based proxy derived from the accumulated cost of NAND operations.

\input{tables/tab_flash_exp_parameter}

To do so, we first use the DT-RAID simulation framework to collect per-tier NAND read and program counts, as summarized earlier in \Cref{fig:flash_breakdown_8disks_raid5}. We then instantiate these counts under specific performance/capacity tier combinations, such as SLC/TLC or SLC/QLC, using representative NAND latency values for each flash mode. \Cref{tab:sim_tier-specs} lists the latency parameters used in this study. These values are selected based on our experience with modern 3D NAND technologies and are consistent with published performance characteristics~\cite{ren2026deviceleveloptimizationtechniquessolidstate}.

We define the flash-time cost of a workload as the total accumulated NAND operation time during trace replay. Each flash read is charged with the tier-dependent read latency \(L_r\), and each flash program is charged with the combined program and erase cost \((L_p + L_e)\). The total flash operation time is therefore
\begin{equation}
\small
T_{\mathrm{flash}} = \sum_{\mathrm{tiers}} \Big( N_{r,\mathrm{tier}} \cdot L_{r,\mathrm{tier}} \;+\; N_{p,\mathrm{tier}} \cdot (L_{p,\mathrm{tier}} + L_{e,\mathrm{tier}}) \Big)
\end{equation}
where \(N_{r,\mathrm{tier}}\) and \(N_{p,\mathrm{tier}}\) denote the total number of flash read and program events attributed to each tier.

This metric provides a controlled proxy for comparing the effective flash cost of different RAID placement policies under identical RAID geometry and workload conditions. It intentionally abstracts away orthogonal factors such as SSD controller implementation, PCIe transfer effects, host-side software overheads, and workload-specific parallelism, allowing us to isolate the contribution of tier-aware RAID placement itself.

%% Section II-B for before add description of figures.
% \Cref{fig:bak_io_data_in_raid} shows the breakdown of I/O activity into data and parity operations for the four write-intensive traces among the 20 largest traces in SNIA IOTTA~\cite{msr_iotta} (Table~\ref{tab:datasets} summarizes these traces, and Section~\ref{sec:exp-method} describes the experimental methodology). Each trace is represented by two bars. The first bar breaks down parity-related activity by update strategy. The second bar shows the overall proportion of data and parity operations in the corresponding trace. We observe that traces with higher fractions of RMW and RCW such as ??? exhibit a larger share of parity-induced I/O activity. For example, \texttt{prxy\_0} which has x-y\% RCM ...has xx\% of parity-related updates. Since parity update introduces additional I/O beyond user data updates, the frequency and locality of partial-stripe updates can materially affect RAID efficiency under write-heavy workloads.


%% Section Evaluation H1
% \Cref{fig:flash_cap_overhead} quantifies the raw-capacity overhead of DT-RAID relative to an all-TLC baseline. Let $\rho$ denote the raw-capacity cost ratio of the performance tier relative to the capacity tier (e.g., $\rho=3$ for SLC/TLC), and let $\phi_{\mathrm{perf}}$ denote the peak fraction of stripe chunks placed in the performance tier during execution. The resulting raw-capacity overhead is

% \begin{equation}
% \small
% \mathrm{Capacity\ Overhead} = (\rho - 1)\phi_{\mathrm{perf}}
% \end{equation}

% For \textit{Static RAID}, parity chunks are permanently placed in the performance tier, so $\phi_{\mathrm{perf}} = M/N$. Under the default 8-disk RAID-5 configuration ($N = 8$, $M = 1$), DT-S therefore incurs a fixed raw-capacity overhead of $25\%$ in the SLC/TLC setting. In contrast, for Dynamic RAID, $\phi_{\mathrm{perf}}$ is determined by the peak promoted stripe footprint observed during execution, yielding a much smaller raw-capacity overhead of $0.6\%$--$5.4\%$ across the evaluated workloads. These results indicate that DT-D achieves most of its tier-steering benefit with substantially lower provisioning costs than DT-S.

==> tables/various_disk_update_type.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Update types count over various disks.}
\label{tab:tier-specs}
\begin{tabular}{l c c c}
\hline
Update Type                    & FSW & RCW    & RMW\\ \hline
4 disks    & 33,647,990 & 23,934,378 & 47,506,112 \\
8 disks & 9,687,869  & 7,392,525 & 60,695,403 \\
16 disks & 645,189 & 6,960,353 & 59,981,902 \\
\hline
\end{tabular}
\end{table}
%SSD-level write amplification ($WA_{SSD}$) & 1.2 & 1.5 \\
